Pipelines and Beyond: Graph Types for ADTs with Futures

Parallel programs are frequently modeled as dependency or cost graphs, which can be used to detect various bugs, or simply to visualize the parallel structure of the code. However, such graphs reflect just one particular execution and are typically constructed in a post-hoc manner. Graph types, which were introduced recently to mitigate this problem, can be assigned statically to a program by a type system and compactly represent the family of all graphs that could result from the program. Unfortunately, prior work is restricted in its treatment of futures, an increasingly common and especially dynamic form of parallelism. In short, each instance of a future must be statically paired with a vertex name. Previously, this led to the restriction that futures could not be placed in collections or be used to construct data structures. Doing so is not a niche exercise: such structures form the basis of numerous algorithms that use forms of pipelining to achieve performance not attainable without futures. All but the most limited of these examples are out of reach of prior graph type systems. In this paper, we propose a graph type system that allows for almost arbitrary combinations of futures and recursive data types. We do so by indexing datatypes with a type-level vertex structure, a codata structure that supplies unique vertex names to the futures in a data structure. We prove the soundness of the system in a parallel core calculus annotated with vertex structures and associated operations. Although the calculus is annotated, this is merely for convenience in defining the type system. We prove that it is possible to annotate arbitrary recursive types with vertex structures, and show using a prototype inference engine that these annotations can be inferred from OCaml-like source code for several complex parallel algorithms.

==> Makefile <==
default: abstract.tex
	pdflatex -interaction nonstopmode main

app: abstract.tex
	cat main.tex | sed 's/\\appfalse/\\apptrue/g' > main-app.tex
	pdflatex -interaction nonstopmode main-app
	bibtex main-app
	pdflatex -interaction nonstopmode main-app
	pdflatex -interaction nonstopmode main-app
	qpdf main-app.pdf --pages . 28-z -- app.pdf

abstract.tex: abstract
	echo "%% DO NOT EDIT THIS FILE-it is produced automatically from the file 'abstract'" > abstract.tex
	cat abstract | sed 's/\*\([^\*]*\)\*/\{\\em \1\}/g' >> abstract.tex

bib: abstract.tex
	pdflatex -interaction nonstopmode main
	bibtex main
	pdflatex -interaction nonstopmode main
	pdflatex -interaction nonstopmode main

clean:
	rm -f *~ *.log *.aux *.bbl *.blg *.brf *.out *.vrb main.pdf


==> dag.tex <==
\section{}\label{sec:graph}

\begin{figure}
  \[
  \begin{array}{l l l}
    \graph & \bnfdef &
    \gvar \bnfalt
    \emptygraph \bnfalt
    \graph \seqcomp \graph \bnfalt
    \graph \parcomp \graph \bnfalt
    \graph \dagor \graph \bnfalt
    \dagrec{\gvar}{\graph}{} \bnfalt
    \leftcomp{\graph}{\vs} \bnfalt
    \touchcomp{\vs} \bnfalt
    \dagpi{\hastycl{\vs}{\vsty}}{\hastycl{\vs}{\vsty}}{\graph} \bnfalt
    \kwtapp{\graph}{\vs}{\vs} \bnfalt\\ & &
    \dagnew{\hastycl{\vs}{\vsty}}{\graph} \bnfalt
    \kwletpair{\vvar}{\vvar}{\vs}{\graph} \bnfalt
    \kwvcase{\vs}{\vvar}{\graph}{\vvar}{\graph}
  \end{array}
  \]
  \caption{Full syntax for graph types.}
  \label{fig:graph-syn}
\end{figure}





\subsection{Graph Type Formation}



%% \begin{lemma}\label{lem:norm-verts}
%%   For all~$\graph$ and all~$n \geq 0$
%%   and all~$\cgraph \in \normgraph{n}{\graph}$,
%%   $\vertsof{\cgraph} \subset \freefut{\graph} \cup \vertices$
%%   where~$\vertices$ is a set of freshly-chosen vertices.
%% \end{lemma}
%% \iffull
%% \begin{proof}
%%   By induction on the derivation of~$\normgraph{n}{\graph}$.
%%   \begin{itemize}
%%   \item $\normgraph{n}{\leftcomp{\graph'}{\vertex}}$.
%%     Then~$\cgraph = \leftcomp{\cgraph'}{\vertex}$
%%     where~$\cgraph' \in \normgraph{n}{\graph'}$.
%%     By induction,~$\vertsof{\cgraph'} \subset \freefut{\graph'} \cup \vertices$.
%%     We have~$\vertsof{\cgraph} = \vertsof{\cgraph'} \cup \{\vertex\}$
%%     and~$\freefut{\graph} = \freefut{\graph'} \cup \{\vertex\}$,
%%     so~$\vertsof{\cgraph} \subset \vertsof{\cgraph'} \cup \{\vertex\}
%%     \subset \freefut{\graph'} \cup \{\vertex\} \cup \vertices =
%%     \freefut{\graph} \cup \vertices$.
%%   \item $\normgraph{n}{\touchcomp{\vertex}}$.
%%     Then~$\vertsof{\cgraph} = \freefut{\graph} = \{\vertex\}$.
%%   \item $\normgraph{n}{\dagnew{\vertex}{\graph'}}$.
%%     Then~$\cgraph \in \normgraph{n}{\sub{\graph'}{\vertex'}{\vertex}}$
%%     where~$\vertex'$ is fresh.
%%     By induction,
%%     \[\vertsof{\cgraph} \subset \freefut{\sub{\graph'}{\vertex'}{\vertex}}
%%     \cup \vertices = \freefut{\graph'} \setminus \{\vertex\} \cup \vertices \cup \vertices'\]
%%     where~$\vertices' = \emptyset$ or~$\vertices' = \{\vertex'\}$.
%%     In either case, all vertices in~$\vertices \cup \vertices'$ are fresh.
%%     We have~$\freefut{\graph} = \freefut{\graph'} \setminus \{\vertex\}$.
%%   \item $\normgraph{n}{\kwtapp{\graph'}{\verts_f}{\verts_t}}$
%%     when~$\gunroll[k]{\graph'} = \dagpi{\verts_f'}{\verts_t'}{\graph''}$.
%%     Then~$\cgraph \in \normgraph{n - k}
%%     {\sub{\sub{\graph''}{\verts_f}{\verts_f'}}{\verts_t}{\verts_t'}}$.
%%     By induction, we have~$\vertsof{\cgraph} \subset
%%     \freefut{\sub{\sub{\graph''}{\verts_f}{\verts_f'}}{\verts_t}{\verts_t'}}
%%     \cup \vertices
%%     = \freefut{\graph''} \setminus (\verts_f' \cup \verts_t') \cup \vertices
%%     \cup \vertices'$
%%     where~$\vertices' \subset \verts_f \cup \verts_t$.
%%     We have~$\freefut{\graph} = \freefut{\graph''}
%%     \setminus (\verts_f' \cup \verts_t') \cup \verts_f \cup \verts_t$.
%%   \end{itemize}
%% \end{proof}
%% \fi

%% \begin{theorem}\label{thm:normalize} For all~$n \geq 0$,
%%   \begin{enumerate}
%%   \item
%%     If~$\dagwf{\ectx}{\uspctx}{\utctx}{\graph}{\graphkind}$
%%     then~$\freefut{\graph} \subset \uspctx$ and~$\graph$ is normalizable at~$n$.
%%   \item
%%     If~$\dagwf{\gvar}{\uspctx}{\utctx}{\graph}{\graphkind}$
%%     then~$\freefut{\graph} \subset \uspctx$
%%     and~$\gsub{\graph}{\dagrec{\gvar}{\dagpi{\verts_f}{\verts_t}{\graph}}{}}{\gvar}$ is normalizable at~$n$.
%%   \end{enumerate}
%% \end{theorem}
%% \iffull
%% \begin{proof}
%%   By lexicographic induction on~$n$ and the type formation derivation.
%% %  derivation of~$\dagwf{\ectx}{\uspctx}{\utctx,\vertex}{\graph}{\graphkind}$.
%%   If~$n = 0$, the result is trivial, so suppose~$n > 0$.
%%   \begin{itemize}
%%   \item \rulename{DW:Var}.
%%     Then~$\gsub{\graph}{\dagrec{\gvar}{\dagpi{\verts_f}{\verts_t}{\graph}}{}}{\gvar}
%%     = \dagrec{\gvar}{\dagpi{\verts_f}{\verts_t}{\graph}}{}$.
%%     Let~$\cgraph \in \normgraph{n}{\dagrec{\gvar}{\dagpi{\verts_f}{\verts_t}{\graph}}{}}$.
%%     We have~$\cgraph \in
%%     \normgraph{n-1}{\gsub{\dagpi{\verts_f}{\verts_t}{\graph}}{\dagrec{\gvar}{\dagpi{\verts_f}{\verts_t}{\graph}}{}}{\gvar}}
%%     \cup \normgraph{n-1}{\dagrec{\gvar}{\dagpi{\verts_f}{\verts_t}{\graph}}{\uctx}}$
%%     and the result follows by induction on~$n$.
%%   \item \rulename{DW:Seq}.
%%     By induction,~$\normgraph{n}{\graph_1}$ and~$\normgraph{n}{\graph_2}$
%%     are well-defined and~$\freefut{\graph_1} \subset \uspctx_1$
%%     and $\freefut{\graph_2} \subset \uspctx_2$.
%%     Let~$\cgraph \in \normgraph{n}{\graph}$.
%%     We have~$\cgraph = \cgraph_1 \seqcomp \cgraph_2$
%%     where~$\cgraph_1 \in \normgraph{n}{\graph_1}$
%%     and~$\cgraph_2 \in \normgraph{n}{\graph_2}$.
%%     By Lemma~\ref{lem:norm-verts},
%%     $\vertsof{\cgraph_1} \subset \uspctx_1 \cup \vertices_1$
%%     and~$\vertsof{\cgraph_2} \subset \uspctx_2 \cup \vertices_2$,
%%     where, without loss of generality,~$\vertices_1$ and~$\vertices_2$ may
%%     be disjoint. The two vertex sets are therefore disjoint and the
%%     graphs may be composed.
%%   \item  \rulename{DW:Or}.
%%     Let~$\cgraph \in \normgraph{n}{\graph_1 \dagor \graph_2}$.
%%     We have either~$\cgraph \in \normgraph{n}{\graph_1}$
%%     or~$\cgraph' \in \normgraph{n}{\graph_2}$.
%%     The result follows from induction in either case.
%%   \item \rulename{DW:RecPi}.
%%     Then $\gunroll[1]{\graph} =
%%     \dagpi{\verts_f}{\verts_t}{\gsub{\graph}
%%       {\dagrec{\gvar}{\dagpi{\verts_f}{\verts_t}{\graph}}{}}{\gvar}}$.
%%     The result follows from  induction.
%%   \item \rulename{DW:Spawn}.
%%     Let~$\cgraph \in \normgraph{n}{\leftcomp{\vertex}{\graph}}$.
%%     We have~$\cgraph = \leftcomp{\cgraph'}{\vertex}$
%%     where~$\cgraph' \in \normgraph{n}{\graph}$.
%%     By induction,~$\cgraph'$ is well-defined
%%     and~$\freefut{\graph} \subset \uspctx \setminus \vertex$.
%%     By Lemma~\ref{lem:norm-verts},~$\vertsof{\cgraph'} \subset \uspctx \setminus
%%     \vertex \cup \vertices$, where without loss of
%%     generality,~$\vertex \not\in \vertices$.
%%     The composition is therefore well-defined.
%%   \item \rulename{DW:New}.
%%     Let~$\cgraph \in \normgraph{n}{\dagnew{\vertex}{\graph}}$.
%%     We have~$\cgraph \in \normgraph{n}{\gsub{\graph}{\vertex'}{\vertex}}$.
%%     By induction, we have that~$\graph$ is normalizable at~$n$
%%     and~$\freefut{\graph} \subset \uspctx$.
%%     By Lemma~\ref{lem:norm-props},~$\cgraph$ is well-defined.
%%     We have~$\freefut{\dagnew{\vertex}{\graph}}
%%     = \freefut{\graph} \setminus \{\vertex\} \subset \uspctx$.
%%   \item \rulename{DW:Pi}.
%%     Then $\gunroll[0]{\graph} =
%%     \dagpi{\verts_f}{\verts_t}{\graph}$ and the result follows from induction.
%%   \item \rulename{DW:App}.
%%     Let~$\cgraph \in \normgraph{n}{\kwtapp{\graph}{\verts_f'}{\verts_t'}}$.
%%     By induction,
%%     $\gunroll[k]{\graph} = \dagpi{\verts_f}{\verts_t}{\graph'}$
%%     and for some~$k$,~$\graph'$
%%     is normalizable at~$n$.
%%     We also have~$\cgraph \in
%%     \normgraph{n-k}{\gsub{\gsub{\graph'}{\verts_f'}{\verts_f}}{\verts_t'}{\verts_t}}$.
%%     By Lemma~\ref{lem:norm-props},~$\cgraph$ is well-defined.
%%   \end{itemize}
%% \end{proof}
%% \else
%% The proof is by lexicographic induction on~$n$ and the
%% appropriate type formation derivation.
%% %derivation of~$\dagwf{\ectx}{\uspctx}{\utctx,\vertex}{\graph}{\graphkind}$.
%% The induction hypothesis on~$n$ is used in the~\rulename{DW:Var} case,
%% where we must reason that~$\dagrec{\gvar}{\dagpi{\verts_f}{\verts_t}{\graph}}{}$
%% is normalizable.
%% %
%% The full proof is in the appendix.
%% \fi


==> fig-graph-eq.tex <==
\begin{figure*}
  \centering
  \def \MathparLineskip {\lineskip=0.43cm}
  \begin{mathpar}
    \Rule{GE-


==> fig-norm.tex <==
\begin{figure*}
    \centering
\begin{mathpar}
\begin{array}{l l l l}
%  \normgraph{0}{\graph} & \defeq & \{\emptygraph\} &\\
%  \normgraph{n}{\emptygraph} & \defeq & \{\emptygraph\} &\\
%  \normgraph{n}{\graph_1 \parcomp \graph_2} & \defeq &
%  \{\graph_1' \parcomp \graph_2' \mid
%  \graph_1' \in \normgraph{n}{\graph_1}, \graph_2' \in \normgraph{n}{\graph_2} &\\
%  \normgraph{n}{\graph_1 \seqcomp \graph_2} & \defeq &
%  \{\graph_1' \seqcomp \graph_2' \mid
%  \graph_1' \in \normgraph{n}{\graph_1}, \graph_2' \in \normgraph{n}{\graph_2} &\\
%  \normgraph{n}{\graph_1 \dagor \graph_2} & \defeq &
%  \normgraph{n}{\graph_1} \cup \normgraph{n}{\graph_2} &\\
  \normgraph{n}{\leftcomp{\graph}{\vs}} & \defeq &
  \{\leftcomp{\graph'}{\vs} \mid \graph' \in \normgraph{n}{\graph}\} &\\
  \normgraph{n}{\touchcomp{\vs}} & \defeq &
  \{\touchcomp{\vs}\} &\\
%  \normgraph{n}{\dagrec{\gvar}{\graph}{\uctx}} & \defeq &
%  \normgraph{n-1}{\gsub{\graph}{\dagrec{\gvar}{\graph}{}}{\gvar}}
%  \cup \normgraph{n-1}{\dagrec{\gvar}{\graph}{\uctx}}
%  &\\
  \normgraph{n}{\dagnew{\hastype{\vs}{\vsty}}{\graph}} & \defeq &
  \normgraph{n}{\gsub{\graph}{\vs'}{\vs}} & \hastype{\vs'}{\vsty}, \vs'\fresh\\
  \normgraph{n}{\kwtapp{\graph}{\verts_f}{\verts_t}} & \defeq &
  \normgraph{n-k}{\gsub{\gsub{\graph'}{\verts_f}{\verts_f'}}{\verts_t}{\verts_t'}} &
  \gunroll[k]{\graph} = \dagpi{\hastype{\vs_f'}{\vsty_f'}}{\hastype{\vs_t'}{\vsty_t'}}{\graph'}\\
  \normgraph{n}{\kwtapp{\graph}{\verts_f}{\verts_t}} & \defeq &
  \emptygraph &
  \gunroll[n]{\graph} \neq \dagpi{\hastype{\vs_f'}{\vsty_f'}}{\hastype{\vs_t'}{\vsty_t'}}{\graph'}

\end{array}
\end{mathpar}
\caption{Additional cases of normalization for futures.}
\label{fig:norm}
\end{figure*}


==> fig-treelike.tex <==
\begin{figure*}
  \small
  \centering
  \def \MathparLineskip {\lineskip=0.43cm}
  \begin{mathpar}
    \Rule{TL:Var}
         {\strut}
         {\vsttree{\vstctx, \vstyvar}{\vstyvar}}
    \and
    \Rule{TL:Vert}
         {\strut}
         {\vsttree{\vstctx}{\kwvty}}
    \and
    \Rule{TL:Pair}
         {\vsttree{\vstctx}{\vsty_1}\\
           \vsttree{\vstctx}{\vsty_2}
         }
         {\vsttree{\vstctx}{\kwprod{\vsty_1}{\vsty_2}}}
    \and
    \Rule{TL:CoRec}
         {\vsttree{\vstctx, \vstyvar}{\vsty}}
         {\vsttree{\vstctx}{\kwvscorec{\vstyvar}{\vsty}}}
  \end{mathpar}
  \caption{Vertex structure type treelike formation.}
  \label{fig:treelike}
\end{figure*}


==> fig-vert-type-verts.tex <==
\begin{figure}
  \[
  \begin{array}{r l l}
    \vstyverts{\kwvty} & \defeq & \{\kwvty\}\\
	\vstyverts{\vsprod{\vsty_1}{\isunav}{\vsty_2}{\isunav}} & \defeq & \emptyset\\
    \vstyverts{\vsprod{\vsty_1}{\isav}{\vsty_2}{\isunav}} & \defeq & 
		  \{\vstyl{\vstyvert} \mid \vstyvert \in \vstyverts{\vsty_1}\}\\
    \vstyverts{\vsprod{\vsty_1}{\isunav}{\vsty_2}{\isav}} & \defeq & 
		  \{\vstyr{\vstyvert} \mid \vstyvert \in \vstyverts{\vsty_2}\}\\
    \vstyverts{\vsprod{\vsty_1}{\isav}{\vsty_2}{\isav}} & \defeq & 
		  \{\vstyl{\vstyvert} \mid \vstyvert \in \vstyverts{\vsty_1}\}
		\cup \{\vstyr{\vstyvert} \mid \vstyvert \in \vstyverts{\vsty_2}\}\\
	\vstyverts{\vstyvar} & \defeq & \emptyset\\
    \vstyverts{\kwvscorec{\vstyvar}{\vsty}} & \defeq & 
		\vstyverts{\vsub{\vsty}{\kwvscorec{\vstyvar}{\vsty}}{\vstyvar}}
  \end{array}
  \]
  \caption{VS type vertex availability.}
  \label{fig:vert-type-verts}
\end{figure}


==> fig-vs-eval.tex <==
\begin{figure*}
  \small
  \centering
  \def \MathparLineskip {\lineskip=0.43cm}
  \begin{mathpar}
    \Rule{UV:Var}
         {\strut}
         {\vseval{\vvar}{\vvar}}
    \and
    \Rule{UV:Path}
         {\strut}
         {\vseval{\vertgen{\vsty}{\genseed}}{\vertgen{\vsty}{\genseed}}}
    \and
    \Rule{UV:Pair}
         {\vseval{\vs_1}{\vs_1'}\\
           \vseval{\vs_2}{\vs_2'}}
         {\vseval{\kwpair{\vs_1}{\vs_2}}{\kwpair{\vs_1'}{\vs_2'}}}
    \and
    \Rule{UV:FstPair}
         {\vseval{\vs}{\kwpair{\vs_1}{\vs_2}}}
         {\vseval{\kwfst{\vs}}{\vs_1}}
    \and
    \Rule{UV:SndPair}
         {\vseval{\vs}{\kwpair{\vs_1}{\vs_2}}}
         {\vseval{\kwsnd{\vs}}{\vs_2}}
    \and
    \Rule{UV:FstNotPair}
         {\vseval{\vs}{\vs'}\\
		\vs' \neq \kwpair{\vs_1}{\vs_2}}
         {\vseval{\kwfst{\vs}}{\kwfst{\vs'}}}
    \and
    \Rule{UV:SndNotPair}
         {\vseval{\vs}{\vs'}\\
		\vs' \neq \kwpair{\vs_1}{\vs_2}}
         {\vseval{\kwsnd{\vs}}{\kwsnd{\vs'}}}
  \end{mathpar}
  \caption{Vertex structure normalization.}
  \label{fig:vs-eval}
\end{figure*}

